LlamaRestTest: Effective REST API Testing with Small Language Models

Modern web services rely heavily on REST APIs, typically documented using the OpenAPI specification. The widespread adoption of this standard has resulted in the development of many black-box testing tools that generate tests based on OpenAPI specifications. Although Large Language Models (LLMs) have shown promising test-generation abilities, their application to REST API testing remains mostly unexplored. We present LlamaRestTest, a novel approach that employs two custom LLMs-created by fine-tuning and quantizing the Llama3-8B model using mined datasets of REST API example values and inter-parameter dependencies-to generate realistic test inputs and uncover inter-parameter dependencies during the testing process by analyzing server responses. We evaluated LlamaRestTest on 12 real-world services (including popular services such as Spotify), comparing it against RESTGPT, a GPT-powered specification-enhancement tool, as well as several state-of-the-art REST API testing tools, including RESTler, MoRest, EvoMaster, and ARAT-RL. Our results demonstrate that fine-tuning enables smaller models to outperform much larger models in detecting actionable parameter-dependency rules and generating valid inputs for REST API testing. We also evaluated different tool configurations, ranging from the base Llama3-8B model to fine-tuned versions, and explored multiple quantization techniques, including 2-bit, 4-bit, and 8-bit integer formats. Our study shows that small language models can perform as well as, or better than, large language models in REST API testing, balancing effectiveness and efficiency. Furthermore, LlamaRestTest outperforms state-of-the-art REST API testing tools in code coverage achieved and internal server errors identified, even when those tools use RESTGPT-enhanced specifications.

==> review.tex <==
Review #827A
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
The paper is focusing on the testing (generating tests) of REST APIs that are accompanied by machine-readable specifications. An LLM-based technique is proposed aiming at identifying valid operation sequences, computing relevant and realistic parameter values and combinations, and generating tests based on the contextual information of the server response messages. The paper reports results based on nine real-world REST services, and five baseline tools showing that the proposed approach significantly outperforms the baselines in terms of code coverage, operation coverage, and number of triggered failures.

Strengths
---------
- Important problem

- Good results

- Interesting approach

Weaknesses
----------
- Lack of comparison with RESTIer

- Assumes complete and exhaustive machine-readable documentation 

- Strong reliance on the returned-related information such as request-related information and 2xx status codes for errors (with an error message).

Comments for authors
--------------------
The paper deals with the automatic testing of REST APIs, which is an important and well-researched topic. The proposed approach is also going further than most of the existing ones by using LLMs to take advantage of the natural language descriptions of the related artifacts, messages, and available information (potentially used when training the LLMs), by using LLMs. Therefore, the proposed method makes a good use of the LLMs capabilities and potential in that context. At the same time, the paper reports results that significantly outperform the related baselines. The conducted experiment seems to be done well providing confidence on the reported results. 

On the negative side though, it seems that the proposed method has some significant limitations. First it assumes a complete and exhaustive specification (machine-readable documentation). Unfortunately, this is not the case for most of the existing APIs and evidently for those APIs that are under development. Unfortunately, the proposed method is also limited in cases of APIs evolutions as the evolution happens before the specification description changes and certainly limited for any use during development. An additional limitation regards the cases where the specification does not include information that is implemented in the APIs (the operation does not exist in the documentation but exists in the API). 

Second, the approach assumes that the API returns relevant request-related information in the HTTP responses and that the 2xx status codes always report successful operation. Again, this assumption is typically not met as most of the APIs do not return relevant information or even worse often return 2xx status codes with error messages. I am afraid, that the first and second limitations are simply too constrained to make this approach applicable and practical.  

The paper compares with many baseline tools. That is good, though one of the most prominent RESTful API testing tools, the RESTler, is not used. Is there any reason for that? Additionally, the paper states (line 799): "These tools were chosen based on their recognition as top-performing solutions in a recent study [20] and their inclusion in the latest industry reports." Please can you indicate what the "latest industry reports" are? Also, the reference [20] studies 8 existing testing tools (RESTler included). Why choosing 5 of them? 

Please note that the number of triggered error codes is an unreelable metric as one can generated multiple failing tests by mutating a failing one (by adding irrelevant values and fields in the request). 

I also feel that reporting the related execution time, model response time, cost, etc of the approach would be good to show the drawbacks and benefits of the proposed method. 

Other comments:

As already stated, a 2xx code is not always successful even if it was designed to be. So what is mentioned in Line 237 is inaccurate. 

Line 368, Line 295, server response messages are almost never precise and informative. Most APIs would not specify the reason why the query is invalid. 

To my knowledge, EvoMaster is primary a white-box tool. Please clarify how the black-box approach of EvoMaster was used and under what. 

Line 561: I believe an LLM does not return well-structured data (cf. hallucinations, and depend on the model temperature). The prompt structure can help making more accurate the LLM responses, but never ensures complete validity. Even if there is a completely fine structure, this may contain invalid data (hallucinations / temperature).

Line 608: While 2xx status codes are intended to indicate valid requests, it might not always be the case. Some APIs return 2xx status codes for invalid requests, but with an error message. 

Line 700 (Mutator): Does the mutator only change routes that can use different methods? Because if changing methods randomly, these might not exist in the API (for that specific route), and result in unnecessary client errors. 

Please indicate what temperature was used for the LLM.

Questions for authors’ response
-------------------------------
1. Is there any reason for not using the RESTler tool?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #827B
===========================================================================
* Updated: Feb 19, 2024, 4:10:31 PM UTC

Overall merit
-------------
1. Reject

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
This work addresses the challenges in REST API testing, particularly the limitations of traditional automated tools which rely heavily on machine-readable API specifications. These tools often miss the nuances of API operation dependencies and realistic input generation. The authors introduce RestTestGPT, an innovative approach using Large Language Models (LLMs) and Chain of Thought (CoT) reasoning to enhance REST API testing. RestTestGPT leverages LLMs to better understand API specifications, generating more effective operation sequences and realistic parameter values. It also incorporates server response messages in its CoT reasoning process for refining test requests. The paper presents an empirical evaluation of RestTestGPT against other state-of-the-art REST testing tools, demonstrating its superior performance in terms of code coverage, operation coverage, and fault detection capabilities.

Strengths
---------
+ Thorough Empirical Evaluation.
+ Addressing Real-world Challenges.

Weaknesses
----------
- Potential for Overfitting.
- Lack of Rigor.
- Chaotic Writing Logic.
- Non-intuitive Presentation.

Comments for authors
--------------------
#### Motivation
- The motivation section could benefit from a clearer articulation of the unique challenges in REST API testing that existing tools fail to address. While the paper mentions the limitations of traditional tools, a more detailed explanation of these limitations would strengthen the argument for the need for a tool like RestTestGPT.

- Right now, the motivation of this paper is not clear. The motivation would be more compelling if backed by empirical evidence or specific examples demonstrating the shortcomings of current REST API testing methods. This could include statistical data or case studies highlighting the failure of existing tools in complex scenarios. The paper could enhance its motivation by discussing the practical implications and relevance of the proposed approach in the context of current industry practices. Demonstrating the alignment of RestTestGPT with industry needs would make a stronger case for its adoption. 

- The paper should more explicitly justify the innovative approach of using LLMs in REST API testing. While the approach is novel, the motivation section should better articulate how this specific technology addresses the identified gaps in the current REST API testing landscape.

#### Soundness

- The paper could benefit from a more robust validation strategy. It should include diverse and complex real-world API scenarios to ensure that the results are not biased towards certain types of APIs or specific settings.

- The evaluation strategy needs to be more comprehensive. The paper should compare RestTestGPT against a wider range of existing tools, under various conditions, to convincingly demonstrate its superiority. This also includes a deeper analysis of cases where RestTestGPT might underperform.

- The paper should address scalability and performance concerns. It's important to demonstrate how RestTestGPT performs in large-scale environments and its resource requirements, as these are critical factors for practical adoption.

- The paper should provide more evidence on the generalizability of the approach. This involves testing RestTestGPT across APIs from different domains and with varying complexity levels to validate its effectiveness broadly.

#### Evaluation

- The evaluation lacks diversity in the selected APIs for testing. It would be beneficial to include a wider range of APIs with varying complexity and from different domains to thoroughly assess the tool's effectiveness.

- The methodology for fault detection needs more clarity. Specifically, how RestTestGPT identifies and categorizes different types of faults compared to existing tools should be detailed.

- The evaluation should address the scalability of the tool. Information on how RestTestGPT performs with large-scale APIs and its computational efficiency is crucial.

- The evaluation lacks details on the reproducibility of the results. Providing access to the datasets, tools, and a clear methodology would enhance the paper's credibility.

- The paper should include statistical analysis to support the claims made. This includes the use of appropriate statistical tests to validate the significance of the observed improvements.


#### Presentation

- Clarity and Structure: The paper is well-structured with a clear introduction, methodology, evaluation, and conclusion. However, some sections could be more concise to enhance readability.

- Figures and Illustrations: While the paper includes helpful figures and illustrations, some of them could be improved in terms of clarity and information conveyance. More detailed captions and a clearer connection to the text would be beneficial.

- The writing style is generally appropriate for an academic paper, but there are instances where the flow could be smoother. Transitions between sections and within paragraphs could be more seamless.

####Additional points

**Concerns Regarding Novelty**: The primary concern lies with the manuscript's exploration of prompt engineering techniques to augment software testing. Although the application of innovative methods to address traditional problems is commendable, the concept of chain-of-thought, as presented, does not offer a novel contribution to the existing body of knowledge. This assertion is supported by the literature, including works like "Make LLM a Testing Expert: Bringing Human-like Interaction to Mobile GUI Testing via Functionality-aware Decisions" and "Fill in the Blank: Context-aware Automated Text Input Generation for Mobile GUI Testing." The manuscript would benefit from a deeper analysis explaining the effectiveness of the proposed approach beyond empirical data.

**Questionable Motivation Example**: The comparison with "Enhancing REST API Testing with NLP Techniques" falls short of convincing. The claim that it suffers from proposed limitations regarding sequence and value generation lacks empirical support from RESTful services, notably absent in Table 2 or Figure 4. This gap undermines the argument's foundation and calls for a more robust data presentation.

**Inadequate Baseline Comparison**: Recent scholarly contributions, such as "Adaptive REST API Testing with Reinforcement Learning" (ASE 2023), "Morest: Model-Based RESTful API Testing with Execution Feedback" (ICSE 2022), and "Combinatorial Testing of RESTful APIs" (ICSE 2022), have not been sufficiently discussed or compared. A comprehensive analysis of these works is essential to establish the proposed method's relevance and innovation.

**Insufficient Evaluation of RESTful Services**: The claim of extensive evaluation in terms of the number of RESTful services tested is not substantiated by the evidence provided. For example, the inclusion of BitBucket as a test service in Morest contrasts with the omission of such an evaluation in the manuscript. This lack of comparative analysis raises questions about the thoroughness of the evaluation process.

**Concerns Over Manuscript Preparation**: There is an observable pattern in the manuscript that suggests significant portions may have been refined using ChatGPT. Although this is a subjective observation without direct evidence, certain indicators, such as the consistent expansion of abbreviations (e.g., "Chain-of-Thought (CoT)", "Large Language Models (LLMs)"), point to the possibility of paragraph-by-paragraph editing, leading to a loss of context and unnatural linkage between sections.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #827C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper introduces an LLM-based approach for REST API testing. The approach focuses on inferring constraints over operations sequences in the execution and generates more likely valid call sequences based on those constraints. The evaluations show results of the proposed approach seem better.

Strengths
---------
+ Addresses a crucial challenge in REST API testing by extracting constraints on operation sequences for valid input generation.
+ Proposes an LLM-based solution, showcasing the potential of leveraging language models in this domain.

Weaknesses
----------
- Requires more detailed explanations regarding contributions and the underlying insights that led to the proposed approach.  
- Missing evaluation of components in the proposed approach
- Insufficient explanation on experiment results
- Issues in the presentation

Comments for authors
--------------------
LLMs demonstrate promising performance in many aspects and it is definitely encouraged to explore using LLMs to test REST APIs. This paper presents an attempt that applies LLMs to REST API testing. However, I have several concerns in the work.

First, the proposed approach is kind of a straw man approach that generates inputs by querying LLMs in a typical way, including identifying valid operation sequence, generating parameter values, etc. I feel it is very necessary to explain the “insight” that leads to this solution. Readers need to know what makes this work and to which extent it works. 

More importantly, those components in the proposed approach need to be evaluated to check if it exactly contributes to final results. In the current evaluation, it only presents overall results, which is insufficient.
 
There are several cases in the experiments showing the proposed approach obtained worse results in terms of coverage and the number found bugs. Investigations are needed to figure out the reasons behind. Even for better results, explanation is needed as well.

The readability issue with Figure 4, possibly due to color choices, needs to be addressed for clearer comprehension.

Questions for authors’ response
-------------------------------
Q1. The evaluation section points out that RestTestGPT always performs worse than other approaches in fault-detection in terms of OMDB. There are also other similar points in the evaluation section. I would like to see case studies in this paper about the reason why RestTestGPT is superior or inferior to traditional approaches, in order to more clearly demonstrate the strengths and weaknesses of RestTestGPT.

Q2. The evaluation section did not explain the reason why "The effect of RestTestGPT is roughly the same as the tools with NLP2REST". Does LLM still have defects in handling some special cases? What cases cannot LLM handle? Hope to see the description of these issues.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #827D
===========================================================================

Decision
--------
1. Reject

Meta-review
-----------
Thank you for submitting a paper to ISSTA 2024.

The reviewers point out that the paper tackles an important problem and addresses real-world challenges. On the other hand, the authors criticize that the approach assumes that complete machine-readable specifications are available and that APIs return request-related information and appropriate status codes at all times. Further, the authors are unsure about the novelty of the approach given that prompt engineering for LLMs is already an active research domain. The authors should compare their work against existing publications in the area. The reviewers also inquire about the effectiveness of the individual components to better understand how and why the approach works.

In total, the reviewers think that this paper is not yet ready for publication at ISSTA 2024.
